IKIWISI: An Interactive Visual Pattern Generator for Evaluating the Reliability of Vision-Language Models Without Ground Truth

We present IKIWISI ("I Know It When I See It"), an interactive visual pattern generator for assessing vision-language models in video object recognition when ground truth is unavailable. IKIWISI transforms model outputs into a binary heatmap where green cells indicate object presence and red cells indicate object absence. This visualization leverages humans' innate pattern recognition abilities to evaluate model reliability. IKIWISI introduces "spy objects": adversarial instances users know are absent, to discern models hallucinating on nonexistent items. The tool functions as a cognitive audit mechanism, surfacing mismatches between human and machine perception by visualizing where models diverge from human understanding. Our study with 15 participants found that users considered IKIWISI easy to use, made assessments that correlated with objective metrics when available, and reached informed conclusions by examining only a small fraction of heatmap cells. This approach not only complements traditional evaluation methods through visual assessment of model behavior with custom object sets, but also reveals opportunities for improving alignment between human perception and machine understanding in vision-language systems.

==> dis25-124 <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{85}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}

\bibitem[\protect\citeauthoryear{??}{Air}{[n.d.]}]%
        {Aira2020}
 \bibinfo{year}{[n.d.]}\natexlab{}.
\newblock \bibinfo{title}{Aira}.
\newblock \bibinfo{howpublished}{\url{https://aira.io/}}.
\newblock


\bibitem[\protect\citeauthoryear{Alsallakh, Hanbury, Hauser, Miksch, and Rauber}{Alsallakh et~al\mbox{.}}{2014}]%
        {alsallakh2014visual}
\bibfield{author}{\bibinfo{person}{Bilal Alsallakh}, \bibinfo{person}{Allan Hanbury}, \bibinfo{person}{Helwig Hauser}, \bibinfo{person}{Silvia Miksch}, {and} \bibinfo{person}{Andreas Rauber}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Visual methods for analyzing probabilistic classification data}.
\newblock \bibinfo{journal}{\emph{IEEE transactions on visualization and computer graphics}} \bibinfo{volume}{20}, \bibinfo{number}{12} (\bibinfo{year}{2014}), \bibinfo{pages}{1703--1712}.
\newblock


\bibitem[\protect\citeauthoryear{Antol, Agrawal, Lu, Mitchell, Batra, Zitnick, and Parikh}{Antol et~al\mbox{.}}{2015}]%
        {antol2015vqa}
\bibfield{author}{\bibinfo{person}{Stanislaw Antol}, \bibinfo{person}{Aishwarya Agrawal}, \bibinfo{person}{Jiasen Lu}, \bibinfo{person}{Margaret Mitchell}, \bibinfo{person}{Dhruv Batra}, \bibinfo{person}{C~Lawrence Zitnick}, {and} \bibinfo{person}{Devi Parikh}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{{VQA}: {Visual} {Question} {Answering}}. In \bibinfo{booktitle}{\emph{Proceedings of the IEEE International Conference on computer vision}}.
\newblock


\bibitem[\protect\citeauthoryear{Behley, Garbade, Milioto, Quenzel, Behnke, Stachniss, and Gall}{Behley et~al\mbox{.}}{2019}]%
        {behley2019iccv}
\bibfield{author}{\bibinfo{person}{J. Behley}, \bibinfo{person}{M. Garbade}, \bibinfo{person}{A. Milioto}, \bibinfo{person}{J. Quenzel}, \bibinfo{person}{S. Behnke}, \bibinfo{person}{C. Stachniss}, {and} \bibinfo{person}{J. Gall}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{{SemanticKITTI: A Dataset for Semantic Scene Understanding of LiDAR Sequences}}. In \bibinfo{booktitle}{\emph{Proc. of the IEEE/CVF International Conf.~on Computer Vision (ICCV)}}.
\newblock


\bibitem[\protect\citeauthoryear{BeMyEyes}{BeMyEyes}{2021}]%
        {BeMyEyes2020}
\bibfield{author}{\bibinfo{person}{BeMyEyes}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \bibinfo{title}{Be My Eyes}.
\newblock \bibinfo{howpublished}{\url{https://www.bemyeyes.com/}}.
\newblock


\bibitem[\protect\citeauthoryear{Billah, Ashok, Porter, and Ramakrishnan}{Billah et~al\mbox{.}}{2017}]%
        {Billah_speeddial}
\bibfield{author}{\bibinfo{person}{Syed~Masum Billah}, \bibinfo{person}{Vikas Ashok}, \bibinfo{person}{Donald~E. Porter}, {and} \bibinfo{person}{I.V. Ramakrishnan}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Speed-Dial: A Surrogate Mouse for Non-Visual Web Browsing}. In \bibinfo{booktitle}{\emph{Proceedings of the 19th International ACM SIGACCESS Conference on Computers and Accessibility}}. \bibinfo{publisher}{ACM}, \bibinfo{address}{3132531}, \bibinfo{pages}{110--119}.
\newblock
\showISBNx{ISBN}
\urldef\tempurl%
\url{https://doi.org/10.1145/3132525.3132531}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Billah and Gauch}{Billah and Gauch}{2015}]%
        {billah2015social}
\bibfield{author}{\bibinfo{person}{Syed~Masum Billah} {and} \bibinfo{person}{Susan Gauch}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Social network analysis for predicting emerging researchers}. In \bibinfo{booktitle}{\emph{2015 7th International Joint Conference on Knowledge Discovery, Knowledge Engineering and Knowledge Management (IC3K)}}, Vol.~\bibinfo{volume}{1}. IEEE, \bibinfo{pages}{27--35}.
\newblock


\bibitem[\protect\citeauthoryear{Billah, Porter, and Ramakrishnan}{Billah et~al\mbox{.}}{2016}]%
        {Billah_sinter}
\bibfield{author}{\bibinfo{person}{Syed~Masum Billah}, \bibinfo{person}{Donald~E. Porter}, {and} \bibinfo{person}{I.~V. Ramakrishnan}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Sinter: low-bandwidth remote access for the visually-impaired}. In \bibinfo{booktitle}{\emph{Proceedings of the Eleventh European Conference on Computer Systems}}. \bibinfo{publisher}{ACM}, \bibinfo{address}{2901335}, \bibinfo{pages}{1--16}.
\newblock
\showISBNx{ISBN}
\urldef\tempurl%
\url{https://doi.org/10.1145/2901318.2901335}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Blanch, Li, Escalera, and Nasrollahi}{Blanch et~al\mbox{.}}{2024}]%
        {blanch2024lidar}
\bibfield{author}{\bibinfo{person}{Miquel~Romero Blanch}, \bibinfo{person}{Zenjie Li}, \bibinfo{person}{Sergio Escalera}, {and} \bibinfo{person}{Kamal Nasrollahi}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{LiDAR-Assisted 3D Human Detection for Video Surveillance}. In \bibinfo{booktitle}{\emph{Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision}}. \bibinfo{pages}{123--131}.
\newblock


\bibitem[\protect\citeauthoryear{Brachman and Levesque}{Brachman and Levesque}{2023}]%
        {brachman2023machines}
\bibfield{author}{\bibinfo{person}{Ronald~J Brachman} {and} \bibinfo{person}{Hector~J Levesque}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{Machines like us: toward AI with common sense}}.
\newblock \bibinfo{publisher}{MIT Press}.
\newblock


\bibitem[\protect\citeauthoryear{Bubeck, Chandrasekaran, Eldan, Gehrke, Horvitz, Kamar, Lee, Lee, Li, Lundberg, et~al\mbox{.}}{Bubeck et~al\mbox{.}}{2023}]%
        {bubeck2023sparks}
\bibfield{author}{\bibinfo{person}{S{\'e}bastien Bubeck}, \bibinfo{person}{Varun Chandrasekaran}, \bibinfo{person}{Ronen Eldan}, \bibinfo{person}{Johannes Gehrke}, \bibinfo{person}{Eric Horvitz}, \bibinfo{person}{Ece Kamar}, \bibinfo{person}{Peter Lee}, \bibinfo{person}{Yin~Tat Lee}, \bibinfo{person}{Yuanzhi Li}, \bibinfo{person}{Scott Lundberg}, {et~al\mbox{.}}} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Sparks of artificial general intelligence: Early experiments with gpt-4}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2303.12712}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Carroll and Olson}{Carroll and Olson}{1988}]%
        {carroll1988mental}
\bibfield{author}{\bibinfo{person}{John~M Carroll} {and} \bibinfo{person}{Judith~Reitman Olson}.} \bibinfo{year}{1988}\natexlab{}.
\newblock \showarticletitle{Mental models in human-computer interaction}.
\newblock \bibinfo{journal}{\emph{Handbook of human-computer interaction}} (\bibinfo{year}{1988}), \bibinfo{pages}{45--65}.
\newblock


\bibitem[\protect\citeauthoryear{Castelo, Rulff, McGowan, Steers, Wu, Chen, Roman, Lopez, Brewer, Zhao, et~al\mbox{.}}{Castelo et~al\mbox{.}}{2023}]%
        {castelo2023argus}
\bibfield{author}{\bibinfo{person}{Sonia Castelo}, \bibinfo{person}{Joao Rulff}, \bibinfo{person}{Erin McGowan}, \bibinfo{person}{Bea Steers}, \bibinfo{person}{Guande Wu}, \bibinfo{person}{Shaoyu Chen}, \bibinfo{person}{Iran Roman}, \bibinfo{person}{Roque Lopez}, \bibinfo{person}{Ethan Brewer}, \bibinfo{person}{Chen Zhao}, {et~al\mbox{.}}} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Argus: Visualization of ai-assisted task guidance in ar}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Chan, Petryk, Gonzalez, Darrell, and Canny}{Chan et~al\mbox{.}}{2023}]%
        {chan2023clair}
\bibfield{author}{\bibinfo{person}{David Chan}, \bibinfo{person}{Suzanne Petryk}, \bibinfo{person}{Joseph~E Gonzalez}, \bibinfo{person}{Trevor Darrell}, {and} \bibinfo{person}{John Canny}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Clair: Evaluating image captions with large language models}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2310.12971}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Chen, Sinavski, H{\"u}nermann, Karnsund, Willmott, Birch, Maund, and Shotton}{Chen et~al\mbox{.}}{2023}]%
        {chen2023driving}
\bibfield{author}{\bibinfo{person}{Long Chen}, \bibinfo{person}{Oleg Sinavski}, \bibinfo{person}{Jan H{\"u}nermann}, \bibinfo{person}{Alice Karnsund}, \bibinfo{person}{Andrew~James Willmott}, \bibinfo{person}{Danny Birch}, \bibinfo{person}{Daniel Maund}, {and} \bibinfo{person}{Jamie Shotton}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Driving with llms: Fusing object-level vector modality for explainable autonomous driving}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2310.01957}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Datta and Dickerson}{Datta and Dickerson}{2023}]%
        {datta2023s}
\bibfield{author}{\bibinfo{person}{Teresa Datta} {and} \bibinfo{person}{John~P Dickerson}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Who's Thinking? A Push for Human-Centered Evaluation of LLMs using the XAI Playbook}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2303.06223}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Feng, Haase-Sch{\"u}tz, Rosenbaum, Hertlein, Glaeser, Timm, Wiesbeck, and Dietmayer}{Feng et~al\mbox{.}}{2020}]%
        {feng2020deep}
\bibfield{author}{\bibinfo{person}{Di Feng}, \bibinfo{person}{Christian Haase-Sch{\"u}tz}, \bibinfo{person}{Lars Rosenbaum}, \bibinfo{person}{Heinz Hertlein}, \bibinfo{person}{Claudius Glaeser}, \bibinfo{person}{Fabian Timm}, \bibinfo{person}{Werner Wiesbeck}, {and} \bibinfo{person}{Klaus Dietmayer}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Deep multi-modal object detection and semantic segmentation for autonomous driving: Datasets, methods, and challenges}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Intelligent Transportation Systems}} \bibinfo{volume}{22}, \bibinfo{number}{3} (\bibinfo{year}{2020}), \bibinfo{pages}{1341--1360}.
\newblock


\bibitem[\protect\citeauthoryear{Fernandez-Manjon and Fernandez-Valmayor}{Fernandez-Manjon and Fernandez-Valmayor}{1998}]%
        {fernandez1998building}
\bibfield{author}{\bibinfo{person}{Baltasar Fernandez-Manjon} {and} \bibinfo{person}{Alfredo Fernandez-Valmayor}.} \bibinfo{year}{1998}\natexlab{}.
\newblock \showarticletitle{Building educational tools based on formal concept analysis}.
\newblock \bibinfo{journal}{\emph{Education and Information Technologies}} \bibinfo{volume}{3}, \bibinfo{number}{3} (\bibinfo{year}{1998}), \bibinfo{pages}{187--201}.
\newblock


\bibitem[\protect\citeauthoryear{Forbes, Holtzman, and Choi}{Forbes et~al\mbox{.}}{2019}]%
        {forbes2019neural}
\bibfield{author}{\bibinfo{person}{Maxwell Forbes}, \bibinfo{person}{Ari Holtzman}, {and} \bibinfo{person}{Yejin Choi}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Do neural language representations learn physical commonsense?}
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1908.02899}} (\bibinfo{year}{2019}).
\newblock


\bibitem[\protect\citeauthoryear{Goodfellow, Pouget-Abadie, Mirza, Xu, Warde-Farley, Ozair, Courville, and Bengio}{Goodfellow et~al\mbox{.}}{2014}]%
        {goodfellow2014generative}
\bibfield{author}{\bibinfo{person}{Ian~J. Goodfellow}, \bibinfo{person}{Jean Pouget-Abadie}, \bibinfo{person}{Mehdi Mirza}, \bibinfo{person}{Bing Xu}, \bibinfo{person}{David Warde-Farley}, \bibinfo{person}{Sherjil Ozair}, \bibinfo{person}{Aaron Courville}, {and} \bibinfo{person}{Yoshua Bengio}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Generative Adversarial Nets}. In \bibinfo{booktitle}{\emph{Advances in Neural Information Processing Systems}}, Vol.~\bibinfo{volume}{27}. \bibinfo{publisher}{Curran Associates, Inc.}, \bibinfo{pages}{2672--2680}.
\newblock


\bibitem[\protect\citeauthoryear{Grier}{Grier}{2015}]%
        {grier2015high}
\bibfield{author}{\bibinfo{person}{Rebecca~A Grier}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{How high is high? A meta-analysis of NASA-TLX global workload scores}. In \bibinfo{booktitle}{\emph{Proceedings of the human factors and ergonomics society annual meeting}}, Vol.~\bibinfo{volume}{59}. Sage Publications Sage CA: Los Angeles, CA, \bibinfo{pages}{1727--1731}.
\newblock


\bibitem[\protect\citeauthoryear{Gupta, Kamath, Kembhavi, and Hoiem}{Gupta et~al\mbox{.}}{2021}]%
        {Gupta2021GPV}
\bibfield{author}{\bibinfo{person}{Tanmay Gupta}, \bibinfo{person}{A. Kamath}, \bibinfo{person}{Aniruddha Kembhavi}, {and} \bibinfo{person}{Derek Hoiem}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Towards General Purpose Vision Systems}.
\newblock \bibinfo{journal}{\emph{ArXiv}}  \bibinfo{volume}{abs/2104.00743} (\bibinfo{year}{2021}).
\newblock


\bibitem[\protect\citeauthoryear{Gupta, Kamath, Kembhavi, and Hoiem}{Gupta et~al\mbox{.}}{2022a}]%
        {gupta2022gpv}
\bibfield{author}{\bibinfo{person}{Tanmay Gupta}, \bibinfo{person}{A. Kamath}, \bibinfo{person}{Aniruddha Kembhavi}, {and} \bibinfo{person}{Derek Hoiem}.} \bibinfo{year}{2022}\natexlab{a}.
\newblock \showarticletitle{Towards General Purpose Vision Systems}.
\newblock \bibinfo{journal}{\emph{Conference of Computer Vision and Pattern Recognition (CVPR)}} (\bibinfo{year}{2022}).
\newblock


\bibitem[\protect\citeauthoryear{Gupta, Kamath, Kembhavi, and Hoiem}{Gupta et~al\mbox{.}}{2022b}]%
        {gupta2022towards}
\bibfield{author}{\bibinfo{person}{Tanmay Gupta}, \bibinfo{person}{Amita Kamath}, \bibinfo{person}{Aniruddha Kembhavi}, {and} \bibinfo{person}{Derek Hoiem}.} \bibinfo{year}{2022}\natexlab{b}.
\newblock \showarticletitle{Towards general purpose vision systems: An end-to-end task-agnostic vision-language architecture}. In \bibinfo{booktitle}{\emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}}. \bibinfo{pages}{16399--16409}.
\newblock


\bibitem[\protect\citeauthoryear{Han, Mitra, and Billah}{Han et~al\mbox{.}}{2024}]%
        {han2024uncovering}
\bibfield{author}{\bibinfo{person}{Chaeeun Han}, \bibinfo{person}{Prasenjit Mitra}, {and} \bibinfo{person}{Syed~Masum Billah}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{Uncovering Human Traits in Determining Real and Spoofed Audio: Insights from Blind and Sighted Individuals}. In \bibinfo{booktitle}{\emph{Proceedings of the CHI Conference on Human Factors in Computing Systems}}. \bibinfo{pages}{1--14}.
\newblock


\bibitem[\protect\citeauthoryear{Hand and Christen}{Hand and Christen}{2018}]%
        {hand2018note}
\bibfield{author}{\bibinfo{person}{David Hand} {and} \bibinfo{person}{Peter Christen}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{A note on using the F-measure for evaluating record linkage algorithms}.
\newblock \bibinfo{journal}{\emph{Statistics and Computing}}  \bibinfo{volume}{28} (\bibinfo{year}{2018}), \bibinfo{pages}{539--547}.
\newblock


\bibitem[\protect\citeauthoryear{Hinterreiter, Ruch, Stitz, Ennemoser, Bernard, Strobelt, and Streit}{Hinterreiter et~al\mbox{.}}{2020}]%
        {hinterreiter2020confusionflow}
\bibfield{author}{\bibinfo{person}{Andreas Hinterreiter}, \bibinfo{person}{Peter Ruch}, \bibinfo{person}{Holger Stitz}, \bibinfo{person}{Martin Ennemoser}, \bibinfo{person}{J{\"u}rgen Bernard}, \bibinfo{person}{Hendrik Strobelt}, {and} \bibinfo{person}{Marc Streit}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{ConfusionFlow: A model-agnostic visualization for temporal analysis of classifier confusion}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Visualization and Computer Graphics}} \bibinfo{volume}{28}, \bibinfo{number}{2} (\bibinfo{year}{2020}), \bibinfo{pages}{1222--1236}.
\newblock


\bibitem[\protect\citeauthoryear{Hohman, Kahng, Pienta, and Chau}{Hohman et~al\mbox{.}}{2018}]%
        {hohman2018visual}
\bibfield{author}{\bibinfo{person}{Fred Hohman}, \bibinfo{person}{Minsuk Kahng}, \bibinfo{person}{Robert Pienta}, {and} \bibinfo{person}{Duen~Horng Chau}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Visual analytics in deep learning: An interrogative survey for the next frontiers}.
\newblock \bibinfo{journal}{\emph{IEEE transactions on visualization and computer graphics}} \bibinfo{volume}{25}, \bibinfo{number}{8} (\bibinfo{year}{2018}), \bibinfo{pages}{2674--2693}.
\newblock


\bibitem[\protect\citeauthoryear{Hoque, Saquib, Billah, and Mueller}{Hoque et~al\mbox{.}}{2020}]%
        {hoque2020toward}
\bibfield{author}{\bibinfo{person}{Md~Naimul Hoque}, \bibinfo{person}{Nazmus Saquib}, \bibinfo{person}{Syed~Masum Billah}, {and} \bibinfo{person}{Klaus Mueller}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Toward Interactively Balancing the Screen Time of Actors Based on Observable Phenotypic Traits in Live Telecast}.
\newblock  \bibinfo{volume}{4}, \bibinfo{number}{CSCW2}, Article \bibinfo{articleno}{154} (\bibinfo{date}{oct} \bibinfo{year}{2020}), \bibinfo{numpages}{18}~pages.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1145/3415225}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Howe and Forbes}{Howe and Forbes}{2008}]%
        {howe2008re}
\bibfield{author}{\bibinfo{person}{Adele~E Howe} {and} \bibinfo{person}{Ryan~D Forbes}.} \bibinfo{year}{2008}\natexlab{}.
\newblock \showarticletitle{Re-considering neighborhood-based collaborative filtering parameters in the context of new data}. In \bibinfo{booktitle}{\emph{Proceedings of the 17th ACM conference on Information and knowledge management}}. \bibinfo{pages}{1481--1482}.
\newblock


\bibitem[\protect\citeauthoryear{Islam and Billah}{Islam and Billah}{2023}]%
        {islam2023spacex}
\bibfield{author}{\bibinfo{person}{Md~Touhidul Islam} {and} \bibinfo{person}{Syed~Masum Billah}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{SpaceX Mag: An Automatic, Scalable, and Rapid Space Compactor for Optimizing Smartphone App Interfaces for Low-Vision Users}.
\newblock \bibinfo{journal}{\emph{Proceedings of the ACM on Interactive, Mobile, Wearable and Ubiquitous Technologies}} \bibinfo{volume}{7}, \bibinfo{number}{2} (\bibinfo{year}{2023}), \bibinfo{pages}{1--36}.
\newblock


\bibitem[\protect\citeauthoryear{Islam, Kabir, Pearce, Reza, and Billah}{Islam et~al\mbox{.}}{2024a}]%
        {islam2024dataset}
\bibfield{author}{\bibinfo{person}{Md~Touhidul Islam}, \bibinfo{person}{Imran Kabir}, \bibinfo{person}{Elena~Ariel Pearce}, \bibinfo{person}{Md~Alimoor Reza}, {and} \bibinfo{person}{Syed~Masum Billah}.} \bibinfo{year}{2024}\natexlab{a}.
\newblock \bibinfo{title}{A Dataset for Crucial Object Recognition in Blind and Low-Vision Individuals' Navigation}.
\newblock
\newblock
\showeprint[arxiv]{2407.16777}~[cs.CV]
\urldef\tempurl%
\url{https://arxiv.org/abs/2407.16777}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Islam, Kabir, Pearce, Reza, and Billah}{Islam et~al\mbox{.}}{2024b}]%
        {islam2024identifying}
\bibfield{author}{\bibinfo{person}{Md~Touhidul Islam}, \bibinfo{person}{Imran Kabir}, \bibinfo{person}{Elene~Ariel Pearce}, \bibinfo{person}{Md~Alimoor Reza}, {and} \bibinfo{person}{Syed~Masum Billah}.} \bibinfo{year}{2024}\natexlab{b}.
\newblock \showarticletitle{Identifying Crucial Objects in Blind and Low-Vision Individuals' Navigation}. In \bibinfo{booktitle}{\emph{The 26th International ACM SIGACCESS Conference on Computers and Accessibility (ASSETS'24)}}. \bibinfo{publisher}{ACM}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1145/3663548.3688538}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Islam, Sojib, Kabir, Amit, Ruhul~Amin, and Billah}{Islam et~al\mbox{.}}{2024c}]%
        {islam2024wheelerdemo}
\bibfield{author}{\bibinfo{person}{Md~Touhidul Islam}, \bibinfo{person}{Noushad Sojib}, \bibinfo{person}{Imran Kabir}, \bibinfo{person}{Ashiqur~Rahman Amit}, \bibinfo{person}{Mohammad Ruhul~Amin}, {and} \bibinfo{person}{Syed~Masum Billah}.} \bibinfo{year}{2024}\natexlab{c}.
\newblock \showarticletitle{Demonstration of Wheeler: A Three-Wheeled Input Device for Usable, Efficient, and Versatile Non-Visual Interaction}. In \bibinfo{booktitle}{\emph{The 37th Annual ACM Symposium on User Interface Software and Technology (UIST Adjunct '24)}}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{Pittsburgh, PA, USA}.
\newblock
\showISBNx{979-8-4007-0718-6/24/10}
\urldef\tempurl%
\url{https://doi.org/10.1145/3672539.3686749}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Islam, Sojib, Kabir, Amit, Ruhul~Amin, and Billah}{Islam et~al\mbox{.}}{2024d}]%
        {islam2024wheeler}
\bibfield{author}{\bibinfo{person}{Md~Touhidul Islam}, \bibinfo{person}{Noushad Sojib}, \bibinfo{person}{Imran Kabir}, \bibinfo{person}{Ashiqur~Rahman Amit}, \bibinfo{person}{Mohammad Ruhul~Amin}, {and} \bibinfo{person}{Syed~Masum Billah}.} \bibinfo{year}{2024}\natexlab{d}.
\newblock \showarticletitle{Wheeler: A Three-Wheeled Input Device for Usable, Efficient, and Versatile Non-Visual Interaction}. In \bibinfo{booktitle}{\emph{The 37th Annual ACM Symposium on User Interface Software and Technology}}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{Pittsburgh, PA, USA}.
\newblock
\showISBNx{979-8-4007-0628-8/24/10}
\urldef\tempurl%
\url{https://doi.org/10.1145/3654777.3676396}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Jia, Gallagher, Saxena, and Chen}{Jia et~al\mbox{.}}{2014}]%
        {jia-3d-stability-pami}
\bibfield{author}{\bibinfo{person}{Zhaoyin Jia}, \bibinfo{person}{Andy Gallagher}, \bibinfo{person}{Ashutosh Saxena}, {and} \bibinfo{person}{Tsuhan Chen}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{3D Reasoning from Blocks to Stability}.
\newblock \bibinfo{journal}{\emph{IEEE Trans PAMI}} (\bibinfo{year}{2014}).
\newblock


\bibitem[\protect\citeauthoryear{Jin and Si}{Jin and Si}{2004}]%
        {jin2004study}
\bibfield{author}{\bibinfo{person}{Rong Jin} {and} \bibinfo{person}{Luo Si}.} \bibinfo{year}{2004}\natexlab{}.
\newblock \showarticletitle{A study of methods for normalizing user ratings in collaborative filtering}. In \bibinfo{booktitle}{\emph{Proceedings of the 27th annual international ACM SIGIR conference on Research and development in information retrieval}}. \bibinfo{pages}{568--569}.
\newblock


\bibitem[\protect\citeauthoryear{Johnson and Johnson}{Johnson and Johnson}{1986}]%
        {johnson1986cooperative}
\bibfield{author}{\bibinfo{person}{Roger~T Johnson} {and} \bibinfo{person}{David~W Johnson}.} \bibinfo{year}{1986}\natexlab{}.
\newblock \showarticletitle{Cooperative learning in the science classroom}.
\newblock \bibinfo{journal}{\emph{Science and children}} \bibinfo{volume}{24}, \bibinfo{number}{2} (\bibinfo{year}{1986}), \bibinfo{pages}{31--32}.
\newblock


\bibitem[\protect\citeauthoryear{Kabir, Reza, and Billah}{Kabir et~al\mbox{.}}{2025}]%
        {kabir2025logicrag}
\bibfield{author}{\bibinfo{person}{Imran Kabir}, \bibinfo{person}{Md~Alimoor Reza}, {and} \bibinfo{person}{Syed Billah}.} \bibinfo{year}{2025}\natexlab{}.
\newblock \showarticletitle{Logic-RAG: Augmenting Large Multimodal Models with Visual-Spatial Knowledge for Road Scene Understanding}. In \bibinfo{booktitle}{\emph{2025 IEEE International Conference on Robotics and Automation (ICRA)}}. IEEE.
\newblock


\bibitem[\protect\citeauthoryear{Kahng, Andrews, Kalro, and Chau}{Kahng et~al\mbox{.}}{2017}]%
        {kahng2017cti}
\bibfield{author}{\bibinfo{person}{Minsuk Kahng}, \bibinfo{person}{Pierre~Y Andrews}, \bibinfo{person}{Aditya Kalro}, {and} \bibinfo{person}{Duen~Horng Chau}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{A cti v is: Visual exploration of industry-scale deep neural network models}.
\newblock \bibinfo{journal}{\emph{IEEE transactions on visualization and computer graphics}} \bibinfo{volume}{24}, \bibinfo{number}{1} (\bibinfo{year}{2017}), \bibinfo{pages}{88--97}.
\newblock


\bibitem[\protect\citeauthoryear{Kamath, Hessel, and Chang}{Kamath et~al\mbox{.}}{2023}]%
        {kamath2023s}
\bibfield{author}{\bibinfo{person}{Amita Kamath}, \bibinfo{person}{Jack Hessel}, {and} \bibinfo{person}{Kai-Wei Chang}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{What's" up" with vision-language models? Investigating their struggle with spatial reasoning}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2310.19785}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Karaoguz and Jensfelt}{Karaoguz and Jensfelt}{2019}]%
        {karaoguz2019object}
\bibfield{author}{\bibinfo{person}{Hakan Karaoguz} {and} \bibinfo{person}{Patric Jensfelt}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Object detection approach for robot grasp detection}. In \bibinfo{booktitle}{\emph{2019 International Conference on Robotics and Automation (ICRA)}}. IEEE, \bibinfo{pages}{4953--4959}.
\newblock


\bibitem[\protect\citeauthoryear{Li, Ouyang, Sheng, Zeng, and Wang}{Li et~al\mbox{.}}{2019}]%
        {li2019gs3d}
\bibfield{author}{\bibinfo{person}{Buyu Li}, \bibinfo{person}{Wanli Ouyang}, \bibinfo{person}{Lu Sheng}, \bibinfo{person}{Xingyu Zeng}, {and} \bibinfo{person}{Xiaogang Wang}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Gs3d: An efficient 3d object detection framework for autonomous driving}. In \bibinfo{booktitle}{\emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}}. \bibinfo{pages}{1019--1028}.
\newblock


\bibitem[\protect\citeauthoryear{Li, Li, Le, Wang, Savarese, and Hoi}{Li et~al\mbox{.}}{2022a}]%
        {li2022lavis}
\bibfield{author}{\bibinfo{person}{Dongxu Li}, \bibinfo{person}{Junnan Li}, \bibinfo{person}{Hung Le}, \bibinfo{person}{Guangsen Wang}, \bibinfo{person}{Silvio Savarese}, {and} \bibinfo{person}{Steven~CH Hoi}.} \bibinfo{year}{2022}\natexlab{a}.
\newblock \showarticletitle{{Lavis}: A library for language-vision intelligence}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2209.09019}} (\bibinfo{year}{2022}).
\newblock


\bibitem[\protect\citeauthoryear{Li, Li, Xiong, and Hoi}{Li et~al\mbox{.}}{2022b}]%
        {li2022blip}
\bibfield{author}{\bibinfo{person}{Junnan Li}, \bibinfo{person}{Dongxu Li}, \bibinfo{person}{Caiming Xiong}, {and} \bibinfo{person}{Steven Hoi}.} \bibinfo{year}{2022}\natexlab{b}.
\newblock \showarticletitle{Blip: Bootstrapping language-image pre-training for unified vision-language understanding and generation}. In \bibinfo{booktitle}{\emph{International Conference on Machine Learning}}. PMLR, \bibinfo{pages}{12888--12900}.
\newblock


\bibitem[\protect\citeauthoryear{Liu, Emerson, and Collier}{Liu et~al\mbox{.}}{2023a}]%
        {liu2023visualspatial}
\bibfield{author}{\bibinfo{person}{Fangyu Liu}, \bibinfo{person}{Guy Emerson}, {and} \bibinfo{person}{Nigel Collier}.} \bibinfo{year}{2023}\natexlab{a}.
\newblock \showarticletitle{Visual spatial reasoning}.
\newblock \bibinfo{journal}{\emph{Transactions of the Association for Computational Linguistics}}  \bibinfo{volume}{11} (\bibinfo{year}{2023}), \bibinfo{pages}{635--651}.
\newblock


\bibitem[\protect\citeauthoryear{Liu, Li, Wu, and Lee}{Liu et~al\mbox{.}}{2023b}]%
        {liu2023visual}
\bibfield{author}{\bibinfo{person}{Haotian Liu}, \bibinfo{person}{Chunyuan Li}, \bibinfo{person}{Qingyang Wu}, {and} \bibinfo{person}{Yong~Jae Lee}.} \bibinfo{year}{2023}\natexlab{b}.
\newblock \showarticletitle{Visual instruction tuning}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2304.08485}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Liu, Li, Wu, and Lee}{Liu et~al\mbox{.}}{2024}]%
        {liu2024visual}
\bibfield{author}{\bibinfo{person}{Haotian Liu}, \bibinfo{person}{Chunyuan Li}, \bibinfo{person}{Qingyang Wu}, {and} \bibinfo{person}{Yong~Jae Lee}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{Visual instruction tuning}.
\newblock \bibinfo{journal}{\emph{Advances in neural information processing systems}}  \bibinfo{volume}{36} (\bibinfo{year}{2024}).
\newblock


\bibitem[\protect\citeauthoryear{Liu, Shi, Cao, Zhu, and Liu}{Liu et~al\mbox{.}}{2017a}]%
        {liu2017analyzing}
\bibfield{author}{\bibinfo{person}{Mengchen Liu}, \bibinfo{person}{Jiaxin Shi}, \bibinfo{person}{Kelei Cao}, \bibinfo{person}{Jun Zhu}, {and} \bibinfo{person}{Shixia Liu}.} \bibinfo{year}{2017}\natexlab{a}.
\newblock \showarticletitle{Analyzing the training processes of deep generative models}.
\newblock \bibinfo{journal}{\emph{IEEE transactions on visualization and computer graphics}} \bibinfo{volume}{24}, \bibinfo{number}{1} (\bibinfo{year}{2017}), \bibinfo{pages}{77--87}.
\newblock


\bibitem[\protect\citeauthoryear{Liu, Wang, Liu, and Zhu}{Liu et~al\mbox{.}}{2017b}]%
        {liu2017towards}
\bibfield{author}{\bibinfo{person}{Shixia Liu}, \bibinfo{person}{Xiting Wang}, \bibinfo{person}{Mengchen Liu}, {and} \bibinfo{person}{Jun Zhu}.} \bibinfo{year}{2017}\natexlab{b}.
\newblock \showarticletitle{Towards better analysis of machine learning models: A visual analytics perspective}.
\newblock \bibinfo{journal}{\emph{Visual Informatics}} \bibinfo{volume}{1}, \bibinfo{number}{1} (\bibinfo{year}{2017}), \bibinfo{pages}{48--56}.
\newblock


\bibitem[\protect\citeauthoryear{Maaz, Rasheed, Khan, and Khan}{Maaz et~al\mbox{.}}{2023}]%
        {maaz2023video}
\bibfield{author}{\bibinfo{person}{Muhammad Maaz}, \bibinfo{person}{Hanoona Rasheed}, \bibinfo{person}{Salman Khan}, {and} \bibinfo{person}{Fahad~Shahbaz Khan}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Video-chatgpt: Towards detailed video understanding via large vision and language models}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2306.05424}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Microsoft}{Microsoft}{2017}]%
        {surface_dial}
\bibfield{author}{\bibinfo{person}{Microsoft}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \bibinfo{title}{Surface Dial}.
\newblock
\newblock
\urldef\tempurl%
\url{https://www.microsoft.com/en-us/surface/accessories/surface-dial}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Newman}{Newman}{2004}]%
        {newman2004coauthorship}
\bibfield{author}{\bibinfo{person}{Mark~EJ Newman}.} \bibinfo{year}{2004}\natexlab{}.
\newblock \showarticletitle{Coauthorship networks and patterns of scientific collaboration}.
\newblock \bibinfo{journal}{\emph{Proceedings of the national academy of sciences}} \bibinfo{volume}{101}, \bibinfo{number}{suppl\_1} (\bibinfo{year}{2004}), \bibinfo{pages}{5200--5205}.
\newblock


\bibitem[\protect\citeauthoryear{Nison}{Nison}{2001}]%
        {nison2001japanese}
\bibfield{author}{\bibinfo{person}{Steve Nison}.} \bibinfo{year}{2001}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{Japanese candlestick charting techniques: a contemporary guide to the ancient investment techniques of the Far East}}.
\newblock \bibinfo{publisher}{Penguin}.
\newblock


\bibitem[\protect\citeauthoryear{Norman and Draper}{Norman and Draper}{1986}]%
        {norman1986user}
\bibfield{author}{\bibinfo{person}{Donald~A Norman} {and} \bibinfo{person}{Stephen~W Draper}.} \bibinfo{year}{1986}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{User centered system design; new perspectives on human-computer interaction}}.
\newblock \bibinfo{publisher}{L. Erlbaum Associates Inc.}
\newblock


\bibitem[\protect\citeauthoryear{OpenAI}{OpenAI}{[n.d.]}]%
        {gptv_system_card}
\bibfield{author}{\bibinfo{person}{OpenAI}.} \bibinfo{year}{[n.d.]}\natexlab{}.
\newblock \bibinfo{title}{GPTV Sysmtem Card}.
\newblock
\newblock
\urldef\tempurl%
\url{https://cdn.openai.com/papers/GPTV_System_Card.pdf}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{OpenAI}{OpenAI}{2023a}]%
        {openai2023gpt4}
\bibfield{author}{\bibinfo{person}{OpenAI}.} \bibinfo{year}{2023}\natexlab{a}.
\newblock \bibinfo{booktitle}{\emph{GPT-4 Technical Report}}.
\newblock
\showeprint[arxiv]{2303.08774v2}
\urldef\tempurl%
\url{https://arxiv.org/abs/2303.08774v2}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{OpenAI}{OpenAI}{2023b}]%
        {openai2023gpt4vsc}
\bibfield{author}{\bibinfo{person}{OpenAI}.} \bibinfo{year}{2023}\natexlab{b}.
\newblock \bibinfo{booktitle}{\emph{GPT-4V(ision) System Card}}.
\newblock
\urldef\tempurl%
\url{https://cdn.openai.com/papers/GPTV_System_Card.pdf}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{OpenAI}{OpenAI}{2023c}]%
        {openai2023gpt4vtwa}
\bibfield{author}{\bibinfo{person}{OpenAI}.} \bibinfo{year}{2023}\natexlab{c}.
\newblock \bibinfo{booktitle}{\emph{GPT-4V(ision) technical work and authors}}.
\newblock
\urldef\tempurl%
\url{https://openai.com/contributions/gpt-4v}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Page, Brin, Motwani, and Winograd}{Page et~al\mbox{.}}{1999}]%
        {page1999pagerank}
\bibfield{author}{\bibinfo{person}{Lawrence Page}, \bibinfo{person}{Sergey Brin}, \bibinfo{person}{Rajeev Motwani}, {and} \bibinfo{person}{Terry Winograd}.} \bibinfo{year}{1999}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{The PageRank citation ranking: Bringing order to the web.}}
\newblock \bibinfo{type}{{T}echnical {R}eport}. \bibinfo{institution}{Stanford infolab}.
\newblock


\bibitem[\protect\citeauthoryear{Paul, Chowdhury, Nicolescu, Nicolescu, and Feil-Seifer}{Paul et~al\mbox{.}}{2021}]%
        {paul2021object}
\bibfield{author}{\bibinfo{person}{Shuvo~Kumar Paul}, \bibinfo{person}{Muhammed~Tawfiq Chowdhury}, \bibinfo{person}{Mircea Nicolescu}, \bibinfo{person}{Monica Nicolescu}, {and} \bibinfo{person}{David Feil-Seifer}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Object detection and pose estimation from rgb and depth data for real-time, adaptive robotic grasping}.
\newblock In \bibinfo{booktitle}{\emph{Advances in Computer Vision and Computational Biology: Proceedings from IPCV'20, HIMS'20, BIOCOMP'20, and BIOENG'20}}. \bibinfo{publisher}{Springer}, \bibinfo{pages}{121--142}.
\newblock


\bibitem[\protect\citeauthoryear{Powers}{Powers}{2020}]%
        {powers2020evaluation}
\bibfield{author}{\bibinfo{person}{David~MW Powers}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Evaluation: from precision, recall and F-measure to ROC, informedness, markedness and correlation}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2010.16061}} (\bibinfo{year}{2020}).
\newblock


\bibitem[\protect\citeauthoryear{Qadir, Islam, and Al-Fuqaha}{Qadir et~al\mbox{.}}{2022}]%
        {qadir2022toward}
\bibfield{author}{\bibinfo{person}{Junaid Qadir}, \bibinfo{person}{Mohammad~Qamar Islam}, {and} \bibinfo{person}{Ala Al-Fuqaha}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Toward accountable human-centered AI: rationale and promising directions}.
\newblock \bibinfo{journal}{\emph{Journal of Information, Communication and Ethics in Society}} \bibinfo{volume}{20}, \bibinfo{number}{2} (\bibinfo{year}{2022}), \bibinfo{pages}{329--342}.
\newblock


\bibitem[\protect\citeauthoryear{Qi, Cun, Zhang, Lei, Wang, Shan, and Chen}{Qi et~al\mbox{.}}{2023}]%
        {qi2023fatezero}
\bibfield{author}{\bibinfo{person}{Chenyang Qi}, \bibinfo{person}{Xiaodong Cun}, \bibinfo{person}{Yong Zhang}, \bibinfo{person}{Chenyang Lei}, \bibinfo{person}{Xintao Wang}, \bibinfo{person}{Ying Shan}, {and} \bibinfo{person}{Qifeng Chen}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Fatezero: Fusing attentions for zero-shot text-based video editing}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2303.09535}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Ren, Amershi, Lee, Suh, and Williams}{Ren et~al\mbox{.}}{2016}]%
        {ren2016squares}
\bibfield{author}{\bibinfo{person}{Donghao Ren}, \bibinfo{person}{Saleema Amershi}, \bibinfo{person}{Bongshin Lee}, \bibinfo{person}{Jina Suh}, {and} \bibinfo{person}{Jason~D Williams}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Squares: Supporting interactive performance analysis for multiclass classifiers}.
\newblock \bibinfo{journal}{\emph{IEEE transactions on visualization and computer graphics}} \bibinfo{volume}{23}, \bibinfo{number}{1} (\bibinfo{year}{2016}), \bibinfo{pages}{61--70}.
\newblock


\bibitem[\protect\citeauthoryear{Riedl}{Riedl}{2019}]%
        {riedl2019human}
\bibfield{author}{\bibinfo{person}{Mark~O Riedl}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Human-centered artificial intelligence and machine learning}.
\newblock \bibinfo{journal}{\emph{Human behavior and emerging technologies}} \bibinfo{volume}{1}, \bibinfo{number}{1} (\bibinfo{year}{2019}), \bibinfo{pages}{33--36}.
\newblock


\bibitem[\protect\citeauthoryear{Sanchez and Wiley}{Sanchez and Wiley}{2009}]%
        {sanchez2009scroll}
\bibfield{author}{\bibinfo{person}{Christopher~A Sanchez} {and} \bibinfo{person}{Jennifer Wiley}.} \bibinfo{year}{2009}\natexlab{}.
\newblock \showarticletitle{To scroll or not to scroll: Scrolling, working memory capacity, and comprehending complex texts}.
\newblock \bibinfo{journal}{\emph{Human Factors}} \bibinfo{volume}{51}, \bibinfo{number}{5} (\bibinfo{year}{2009}), \bibinfo{pages}{730--738}.
\newblock


\bibitem[\protect\citeauthoryear{Simons and Levin}{Simons and Levin}{1997}]%
        {simons1997change}
\bibfield{author}{\bibinfo{person}{Daniel~J Simons} {and} \bibinfo{person}{Daniel~T Levin}.} \bibinfo{year}{1997}\natexlab{}.
\newblock \showarticletitle{Change blindness}.
\newblock \bibinfo{journal}{\emph{Trends in cognitive sciences}} \bibinfo{volume}{1}, \bibinfo{number}{7} (\bibinfo{year}{1997}), \bibinfo{pages}{261--267}.
\newblock


\bibitem[\protect\citeauthoryear{Thrush, Jiang, Bartolo, Singh, Williams, Kiela, and Ross}{Thrush et~al\mbox{.}}{2022}]%
        {thrush2022winoground}
\bibfield{author}{\bibinfo{person}{Tristan Thrush}, \bibinfo{person}{Ryan Jiang}, \bibinfo{person}{Max Bartolo}, \bibinfo{person}{Amanpreet Singh}, \bibinfo{person}{Adina Williams}, \bibinfo{person}{Douwe Kiela}, {and} \bibinfo{person}{Candace Ross}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Winoground: Probing vision and language models for visio-linguistic compositionality}. In \bibinfo{booktitle}{\emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}}. \bibinfo{pages}{5238--5248}.
\newblock


\bibitem[\protect\citeauthoryear{Todorovic}{Todorovic}{2008}]%
        {todorovic2008gestalt}
\bibfield{author}{\bibinfo{person}{Dejan Todorovic}.} \bibinfo{year}{2008}\natexlab{}.
\newblock \showarticletitle{Gestalt principles}.
\newblock \bibinfo{journal}{\emph{Scholarpedia}} \bibinfo{volume}{3}, \bibinfo{number}{12} (\bibinfo{year}{2008}), \bibinfo{pages}{5345}.
\newblock


\bibitem[\protect\citeauthoryear{Treisman}{Treisman}{1985}]%
        {treisman1985preattentive}
\bibfield{author}{\bibinfo{person}{Anne Treisman}.} \bibinfo{year}{1985}\natexlab{}.
\newblock \showarticletitle{Preattentive processing in vision}.
\newblock \bibinfo{journal}{\emph{Computer vision, graphics, and image processing}} \bibinfo{volume}{31}, \bibinfo{number}{2} (\bibinfo{year}{1985}), \bibinfo{pages}{156--177}.
\newblock


\bibitem[\protect\citeauthoryear{Treisman and Gelade}{Treisman and Gelade}{1980}]%
        {treisman1980feature}
\bibfield{author}{\bibinfo{person}{Anne~M Treisman} {and} \bibinfo{person}{Garry Gelade}.} \bibinfo{year}{1980}\natexlab{}.
\newblock \showarticletitle{A feature-integration theory of attention}.
\newblock \bibinfo{journal}{\emph{Cognitive psychology}} \bibinfo{volume}{12}, \bibinfo{number}{1} (\bibinfo{year}{1980}), \bibinfo{pages}{97--136}.
\newblock


\bibitem[\protect\citeauthoryear{Wang, Bochkovskiy, and Liao}{Wang et~al\mbox{.}}{2023a}]%
        {wang2023yolov7}
\bibfield{author}{\bibinfo{person}{Chien-Yao Wang}, \bibinfo{person}{Alexey Bochkovskiy}, {and} \bibinfo{person}{Hong-Yuan~Mark Liao}.} \bibinfo{year}{2023}\natexlab{a}.
\newblock \showarticletitle{YOLOv7: Trainable bag-of-freebies sets new state-of-the-art for real-time object detectors}. In \bibinfo{booktitle}{\emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}}. \bibinfo{pages}{7464--7475}.
\newblock


\bibitem[\protect\citeauthoryear{Wang, Zhang, Wang, Cao, Zhou, Zhang, Liu, Fan, and Tian}{Wang et~al\mbox{.}}{2023b}]%
        {wang2023human}
\bibfield{author}{\bibinfo{person}{Liuping Wang}, \bibinfo{person}{Zhan Zhang}, \bibinfo{person}{Dakuo Wang}, \bibinfo{person}{Weidan Cao}, \bibinfo{person}{Xiaomu Zhou}, \bibinfo{person}{Ping Zhang}, \bibinfo{person}{Jianxing Liu}, \bibinfo{person}{Xiangmin Fan}, {and} \bibinfo{person}{Feng Tian}.} \bibinfo{year}{2023}\natexlab{b}.
\newblock \showarticletitle{Human-centered design and evaluation of AI-empowered clinical decision support systems: a systematic review}.
\newblock \bibinfo{journal}{\emph{Frontiers in Computer Science}}  \bibinfo{volume}{5} (\bibinfo{year}{2023}), \bibinfo{pages}{1187299}.
\newblock


\bibitem[\protect\citeauthoryear{Ward, Grinstein, and Keim}{Ward et~al\mbox{.}}{2010}]%
        {ward2010interactive}
\bibfield{author}{\bibinfo{person}{Matthew~O Ward}, \bibinfo{person}{Georges Grinstein}, {and} \bibinfo{person}{Daniel Keim}.} \bibinfo{year}{2010}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{Interactive Data Disualization: Foundations, Techniques, and Applications}}.
\newblock \bibinfo{publisher}{CRC Press}.
\newblock


\bibitem[\protect\citeauthoryear{West, Lu, Dziri, Brahman, Li, Hwang, Jiang, Fisher, Ravichander, Chandu, et~al\mbox{.}}{West et~al\mbox{.}}{2023}]%
        {west2023generative}
\bibfield{author}{\bibinfo{person}{Peter West}, \bibinfo{person}{Ximing Lu}, \bibinfo{person}{Nouha Dziri}, \bibinfo{person}{Faeze Brahman}, \bibinfo{person}{Linjie Li}, \bibinfo{person}{Jena~D Hwang}, \bibinfo{person}{Liwei Jiang}, \bibinfo{person}{Jillian Fisher}, \bibinfo{person}{Abhilasha Ravichander}, \bibinfo{person}{Khyathi Chandu}, {et~al\mbox{.}}} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{THE GENERATIVE AI PARADOX:“What It Can Create, It May Not Understand”}. In \bibinfo{booktitle}{\emph{The Twelfth International Conference on Learning Representations}}.
\newblock


\bibitem[\protect\citeauthoryear{Xie, Yu, Zhang, Billah, Lee, and Carroll}{Xie et~al\mbox{.}}{2025}]%
        {xie2025beyond}
\bibfield{author}{\bibinfo{person}{Jingyi Xie}, \bibinfo{person}{Rui Yu}, \bibinfo{person}{He Zhang}, \bibinfo{person}{Syed~Masum Billah}, \bibinfo{person}{Sooyeon Lee}, {and} \bibinfo{person}{John~M Carroll}.} \bibinfo{year}{2025}\natexlab{}.
\newblock \showarticletitle{Beyond Visual Perception: Insights from Smartphone Interaction of Visually Impaired Users with Large Multimodal Models}. In \bibinfo{booktitle}{\emph{Proceedings of the 2025 CHI Conference on Human Factors in Computing Systems}}. \bibinfo{pages}{1--17}.
\newblock


\bibitem[\protect\citeauthoryear{Xie, Yu, Zhang, Lee, Billah, and Carroll}{Xie et~al\mbox{.}}{2024}]%
        {xie2024emerging}
\bibfield{author}{\bibinfo{person}{Jingyi Xie}, \bibinfo{person}{Rui Yu}, \bibinfo{person}{He Zhang}, \bibinfo{person}{Sooyeon Lee}, \bibinfo{person}{Syed~Masum Billah}, {and} \bibinfo{person}{John~M Carroll}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{Emerging practices for large multimodal model (lmm) assistance for people with visual impairments: Implications for design}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2407.08882}} (\bibinfo{year}{2024}).
\newblock


\bibitem[\protect\citeauthoryear{Yang, Jia, Li, and Yan}{Yang et~al\mbox{.}}{2023}]%
        {yang2023survey}
\bibfield{author}{\bibinfo{person}{Zhenjie Yang}, \bibinfo{person}{Xiaosong Jia}, \bibinfo{person}{Hongyang Li}, {and} \bibinfo{person}{Junchi Yan}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{A survey of large language models for autonomous driving}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2311.01043}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Yuksekgonul, Bianchi, Kalluri, Jurafsky, and Zou}{Yuksekgonul et~al\mbox{.}}{2022}]%
        {yuksekgonul2022and}
\bibfield{author}{\bibinfo{person}{Mert Yuksekgonul}, \bibinfo{person}{Federico Bianchi}, \bibinfo{person}{Pratyusha Kalluri}, \bibinfo{person}{Dan Jurafsky}, {and} \bibinfo{person}{James Zou}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{When and why vision-language models behave like bag-of-words models, and what to do about it}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2210.01936}}  \bibinfo{volume}{5} (\bibinfo{year}{2022}).
\newblock


\bibitem[\protect\citeauthoryear{Zhang, Falletta, Xie, Yu, Lee, Billah, and Carroll}{Zhang et~al\mbox{.}}{2025}]%
        {zhang2025enhancing}
\bibfield{author}{\bibinfo{person}{He Zhang}, \bibinfo{person}{Nicholas~J Falletta}, \bibinfo{person}{Jingyi Xie}, \bibinfo{person}{Rui Yu}, \bibinfo{person}{Sooyeon Lee}, \bibinfo{person}{Syed~Masum Billah}, {and} \bibinfo{person}{John~M Carroll}.} \bibinfo{year}{2025}\natexlab{}.
\newblock \showarticletitle{Enhancing the Travel Experience for People with Visual Impairments through Multimodal Interaction: NaviGPT, A Real-Time AI-Driven Mobile Navigation System}. In \bibinfo{booktitle}{\emph{Companion Proceedings of the 2025 ACM International Conference on Supporting Group Work}}. \bibinfo{pages}{29--35}.
\newblock


\bibitem[\protect\citeauthoryear{Zhang, Wang, Molino, Li, and Ebert}{Zhang et~al\mbox{.}}{2018b}]%
        {zhang2018manifold}
\bibfield{author}{\bibinfo{person}{Jiawei Zhang}, \bibinfo{person}{Yang Wang}, \bibinfo{person}{Piero Molino}, \bibinfo{person}{Lezhi Li}, {and} \bibinfo{person}{David~S Ebert}.} \bibinfo{year}{2018}\natexlab{b}.
\newblock \showarticletitle{Manifold: A model-agnostic framework for interpretation and diagnosis of machine learning models}.
\newblock \bibinfo{journal}{\emph{IEEE transactions on visualization and computer graphics}} \bibinfo{volume}{25}, \bibinfo{number}{1} (\bibinfo{year}{2018}), \bibinfo{pages}{364--373}.
\newblock


\bibitem[\protect\citeauthoryear{Zhang, Isola, Efros, Shechtman, and Wang}{Zhang et~al\mbox{.}}{2018a}]%
        {zhang2018unreasonable}
\bibfield{author}{\bibinfo{person}{Richard Zhang}, \bibinfo{person}{Phillip Isola}, \bibinfo{person}{Alexei~A Efros}, \bibinfo{person}{Eli Shechtman}, {and} \bibinfo{person}{Oliver Wang}.} \bibinfo{year}{2018}\natexlab{a}.
\newblock \showarticletitle{The unreasonable effectiveness of deep features as a perceptual metric}. In \bibinfo{booktitle}{\emph{Proceedings of the IEEE conference on computer vision and pattern recognition}}. \bibinfo{pages}{586--595}.
\newblock


\bibitem[\protect\citeauthoryear{Zhou, Liu, Zagar, Yurtsever, and Knoll}{Zhou et~al\mbox{.}}{2023}]%
        {zhou2023vision}
\bibfield{author}{\bibinfo{person}{Xingcheng Zhou}, \bibinfo{person}{Mingyu Liu}, \bibinfo{person}{Bare~Luka Zagar}, \bibinfo{person}{Ekim Yurtsever}, {and} \bibinfo{person}{Alois~C Knoll}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{Vision language models in autonomous driving and intelligent transportation systems}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2310.14414}} (\bibinfo{year}{2023}).
\newblock


\bibitem[\protect\citeauthoryear{Zimmerman, Forlizzi, and Evenson}{Zimmerman et~al\mbox{.}}{2007}]%
        {research_through_design}
\bibfield{author}{\bibinfo{person}{John Zimmerman}, \bibinfo{person}{Jodi Forlizzi}, {and} \bibinfo{person}{Shelley Evenson}.} \bibinfo{year}{2007}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{Research through Design as a Method for Interaction Design Research in HCI}}.
\newblock \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{493–502}.
\newblock
\showISBNx{9781595935939}
\urldef\tempurl%
\url{https://doi.org/10.1145/1240624.1240704}
\showURL{%
\tempurl}


\end{thebibliography}


==> sections/3.inception.tex <==
\section{Design Inception}
\label{sec:inception}

The inception of \sysname{} was directly inspired by a request from members of a local chapter of the National Federation of the Blind (NFB). 
These individuals, who are intimately familiar with the challenges faced by people with visual impairments, reached out to our research team with a unique problem: they needed a way for sighted companions of blind individuals—who are often non-experts in AI technology—to effectively evaluate the reliability and performance of large, multi-modal AI models (LMMs) designed to assist blind users.

The NFB members shared their experiences with existing AI-powered apps like Seeing AI~\cite{SeeingAI2020}, which, while helpful, often fall short in real-time applications. 
These apps typically require users to take a photo and wait for a description, which is impractical for navigation or other immediate needs. 
As a result, many blind users still rely on services like Aira~\cite{Aira2020} or Be My Eyes~\cite{BeMyEyes2020}, which connect them with remote sighted assistants. 
The NFB members, however, envisioned a more autonomous solution—one where large, multi-modal models like GPT-4 could provide real-time object detection tailored to specific, user-defined needs.

During our discussions, the NFB members emphasized the crucial role of sighted companions in their daily lives. 
These companions, who often have a deep understanding of the specific challenges faced by blind individuals, play a key role in interpreting and evaluating the outputs of AI systems. 
However, these companions are not typically experts in AI and thus require tools that are both intuitive and effective in assessing the performance of such models.

This need for a user-friendly, accessible evaluation tool for non-experts led us to develop \sysname{}. 
We recognized that while faster multi-object detectors like YOLOv7~\cite{wang2023yolov7} could detect predefined objects, the real challenge was to enable the detection of multiple, user-selected objects in real-time—something that traditional models struggle with. Furthermore, evaluating the performance of these models, especially in the absence of ground truth data, posed a significant challenge.

\sysname{} was thus designed as a solution that leverages the human visual perception and contextual understanding of sighted users. 
The tool uses a simple, intuitive heatmap to visually represent the performance of LMMs across selected objects and scenarios, enabling these non-expert users to detect patterns and anomalies quickly. 
This visual approach allows users to make informed judgments about the reliability and relevance of AI models in real-world contexts.







% The idea for \sysname{} originated when members of a local chapter of the National Federation of the Blind (NFB) contacted one of the authors of our research team.
% %
% They inquired about the feasibility of designing a smartphone app to describe objects in a scene captured by the smartphone's live camera in real-time.
% %
% The NFB members mentioned that they used several AI-powered apps, such as Seeing AI~\cite{SeeingAI2020}, but none worked in real-time – users needed to take a photo and wait for some time to get the image description. 
% For real-time assistance, they still relied on remote-sighted assistants like Aira~\cite{Aira2020} or Be My Eyes~\cite{BeMyEyes2020} services.
% % 
% They were very excited about the capabilities of large, multi-modal models like GPT-4 and were curious whether it would be technologically possible to receive real-time object descriptions via these new types of AIs. 
% Upon further conversation, it turned out that they had a particular use case in mind – they wanted AI to subscribe to a small subset of objects critical for their navigation and report the appearance or disappearance of these objects in real-time. 
% Such objects include stairs, road signs, barrier posts, and overhanging tree branches that their canes usually do not pick up; or objects like pet waste that they do not want their canes to pick up.
% % 
% We identified that faster multi-object detectors like YOLOv7~\cite{wang2023yolov7} could work but quickly realized that the problem was, in fact,
% \textit{detecting multiple, user-selected objects} rather than detecting a set of predefined objects. 
% For example, YOLOv7~\cite{wang2023yolov7} cannot detect pet waste by default. 
% This led us to explore large, open-vocabulary, general-purpose vision-language models like GPV-1 and GPT-4, where users can ask the model to detect an object by natural language prompt.
% The idea was to detect user-selected objects 
% in each video frame. 


% However, there were two issues with this approach: 1) the responses were not in real-time
% %~\redcolor{REZA: confirm the frame rate of GPV/GPT}
% ; 2) there was no easy way to compare the detection performance of different models on the user-selected objects.
% To address the first problem, we prefetched the responses from different models and stored them in a cache for a video. 
% However, to address the second problem, we needed to design a new diagnostic tool that did not rely on human-annotated ground truth data yet provided a reasonable estimate of the models' performance. This led to the design of \sysname{}.






==> sections/old.tex <==



\subsection{\sysname{} as a Window into AI’s Commonsense Gaps}

While \sysname{} was initially designed as a usability interface to facilitate user-friendly evaluation of vision-language models (VLMs), our study results suggest that it also operates as a cognitive audit tool, surfacing and interrogating the boundary between human commonsense reasoning and machine perception. 
In real-world, query-driven scenarios, users rely on commonsense expectations of what should be visually salient. 
Our findings show that \sysname{} enables users to intuitively identify mismatches between these expectations and the model’s behavior, without needing to inspect the entire performance space.

For instance, participants frequently used high-level visual patterns (e.g., uni-color rows, checkered patterns) to make judgments with minimal effort (Sec.~\ref{subsec:role_of_patterns}). 
Many participants confidently assessed a model’s reliability after examining just a fraction of the heatmap cells, suggesting that \sysname{} taps into users’ internal mental models of object continuity and co-occurrence (Results \textbf{R6–R9} in Sec.~\ref{subsec:role_of_patterns}). 
Particularly, users penalized models showing inconsistent recognition across visually similar frames, which they saw as a violation of physical plausibility and pattern stability (Sec.~\ref{subsec:inter-frame}). 
Conversely, they showed tolerance for model failures involving objects they deemed visually ambiguous or contextually improbable—an indication that participants were not merely evaluating correctness, but appropriateness in context.

Moreover, the tool's incorporation of ``spy" objects—unlikely to appear in any frame—allowed users to test a model’s ability to infer absence, further showcasing \sysname{}’s role in enabling hypothesis-driven scrutiny of model behavior. 
This investigative use aligns with the goals of cognitive auditing: identifying edge cases, implicit assumptions, and model blind spots in a structured, user-driven manner.

Ultimately, \sysname{} does more than present binary outputs — it scaffolds a process through which users explore and reflect on the boundaries of AI understanding. 
This interpretation situates \sysname{} within broader HCI and AI interpretability conversations, highlighting its potential not only as a diagnostic interface but also as a means of promoting transparency, alignment, and critical reflection in human-AI collaboration.









\subsection{\sysname{} and the Future of Human-in-the-Loop AI Evaluation}

\subsubsection{\sysname{} as a Human-Centered AI Evaluation Tool}

\sysname{} addresses the challenge of evaluating AI systems where ground truth is limited or absent—particularly in dynamic, real-world scenarios like autonomous navigation or assistive technology. Traditional metrics depend on predefined benchmarks, but these often fail to capture contextual nuances or rare events.

To overcome these limitations, \sysname{} adopts a human-centered approach that leverages human visual perception and commonsense reasoning. Through its simple yet powerful heatmap interface, evaluators can detect trends and anomalies that are not readily visible through quantitative metrics. This enables more nuanced judgment in ambiguous or edge-case situations.

Such interpretability and user-in-the-loop evaluation align with broader calls for fairness, accountability, and transparency in AI design~\cite{riedl2019human, sperrle2021survey, vaughan2021human, zhou2018human}. \sysname{} fosters these goals by empowering users to engage directly with model outputs and critically assess AI reliability in practical contexts.

\subsubsection{\sysname{} as a Task-Specific LMM Prompting Framework}

As large, multi-modal models advance into domains such as text-to-video generation, task-specific evaluations become increasingly necessary. \sysname{}’s framework can be adapted by replacing \textit{objects} with \textit{phrases} (e.g., \textit{Shining Sun}, \textit{Smiling Baby}) extracted from text prompts. Users can then track whether these visual elements appear consistently and accurately across video frames.

This adaptation enables a structured, frame-by-frame evaluation of LMMs’ ability to convert language into coherent visual content~\cite{khachatryan2023text2video, guo2023animatediff, huang2024free}, supporting both qualitative inspection and domain-specific benchmarking.

\subsubsection{\sysname{} in Promoting User Agency}

\sysname{} enhances user agency by making LMM evaluation accessible to non-experts through an intuitive interface. This democratization dismantles barriers that often limit evaluation to technical communities. Users can explore model behavior, assess performance based on their own context, and provide meaningful feedback.

Such inclusive evaluation not only broadens participation but also contributes to better model development. As users identify strengths, limitations, and misalignments, their insights help refine models for specific use cases—ensuring that AI development remains grounded in diverse, real-world needs.

\subsubsection{\sysname{} as a Complement to Automated Evaluations}

While automated metrics like $F_1$-score are essential, they require structured ground truth data—something not always available in practical applications~\cite{gptv_system_card}. \sysname{} complements such metrics by enabling users to evaluate models through selective inspection of a few objects and frames.

Despite this minimal input, participant ratings in our study closely aligned with models’ $F_1$ scores across full datasets (Sec.~\ref{subsec:all_org_model_ratings}). This suggests that \sysname{} offers a lightweight yet reliable framework for assessing model reliability when quantitative benchmarking is constrained.
















\subsection{\sysname{} as a Human-Centered AI Evaluation Tool}

\sysname{} addresses the critical challenge of evaluating AI systems in scenarios where ground truth data is either unavailable or insufficient. 
Traditional evaluation metrics rely heavily on predefined benchmarks and ground truth labels to measure an AI model’s accuracy and performance. 
However, in many real-world applications—such as dynamic scene analysis, autonomous navigation, and assisting people with visual impairments—such ground truth data may be either infeasible to obtain or too restrictive to capture the complexity of the environment.

To overcome these limitations, \sysname{} introduces a human-centered approach to AI evaluation that leverages the unique strengths of human perception, domain knowledge, and intuition. 
By providing a simple yet powerful visual representation, the system enables evaluators to discern patterns, trends, and anomalies in the model’s outputs that may not be immediately apparent through quantitative metrics alone. T
his qualitative assessment method allows for a richer, more nuanced understanding of model performance, particularly in edge cases or ambiguous situations where the model’s decision-making process must align with human expectations.

This approach is increasingly recognized as essential in the broader context of AI development, where fairness, accountability, interpretability, and transparency are becoming critical pillars of responsible AI design~\cite{riedl2019human, sperrle2021survey, vaughan2021human, zhou2018human}. 
\sysname{} contributes to this discourse by empowering users to engage directly with the AI model’s outputs, fostering a deeper understanding of how the model operates in complex, real-world environments. 
This not only aids in identifying potential biases or errors in the model but also supports the creation of AI systems that are more aligned with human values and expectations.

Moreover, the dual evaluation approach facilitated by \sysname{}---combining qualitative insights from human evaluators with traditional quantitative metrics---offers a more holistic view of AI model performance. 
It ensures that models are not only accurate in a statistical sense but also reliable and trustworthy in practical, real-world applications. 
This alignment between algorithmic accuracy and human expectations is crucial for the broader acceptance and ethical deployment of AI systems in society. 
As AI continues to permeate critical sectors such as healthcare, transportation, and security, tools like \sysname{} will play a vital role in ensuring these systems operate in a manner that is both effective and just.



% \subsection{{The Role of Context in Perceived Reliability}} 
% Reliability in LMMs extends beyond mere accuracy metrics to encompass context-sensitive interpretations of data. 
% Our study findings show that when the potential use case of an LMM is sensitive, such as blind navigation assistance or automated driving---mistakes in essential objects like cars and white canes can significantly affect perceived reliability (Sec.\ref{subsec:role_of_contect}).
% %
% Such context-dependent evaluations reveal a gap in traditional metrics like F-scores and accuracy and LMM-providers' metrics such as refusal to generate harmful or hateful content~\cite{gptv_system_card}.
% These metrics fail to capture the nuanced expectations users have from these models based on their real-world applications.

% A user-centric evaluation approach, as demonstrated by \sysname{}, can bridge this gap by aligning model assessment with user expectations and application-specific requirements. 
% % 
% Through \sysname{}, users directly interact with model outputs, providing insights into the accuracy and contextual appropriateness of the results.








% \subsection{{\sysname{} as a Task-Specific LMM Prompting Framework}}
% % 
% As LMMs continue to advance, tools like \sysname{} are crucial for domain-specific evaluations.
% For example, in text-to-video generation tasks, assessing a model's capability to translate textual descriptions into video accurately requires an in-depth understanding of the text and the generated visuals~\cite{khachatryan2023text2video, guo2023animatediff, huang2024free}.
% %
% \sysname{} could offer a structured approach for prompting such LMMs.
% One could potentially substitute \emph{`objects'} (e.g., White Cane, Person, Car) with \emph{`phrases'} (e.g., `Shining Sun,' `Smiling Baby,' `Floating Astronaut') from the text, 
% enabling users to gauge the model's frame-by-frame accuracy in a video generation task.



\subsection{{\sysname{} as a Task-Specific LMM Prompting Framework}}
As large, multi-modal AI models (LMMs) extend into domains like text-to-video generation, evaluating their performance requires more than just accuracy metrics. 
%
By adapting \sysname{}'s framework replacing \textit{objects} with \textit{phrases} from text prompts---such as \textit{Shining Sun'} or \textit{Smiling Baby'}---users can track these specific elements across video frames.
%
This enables a granular, context-sensitive evaluation of the model’s ability to translate text into accurate and coherent visuals, ensuring consistency and relevance in the generated content~\cite{khachatryan2023text2video, guo2023animatediff, huang2024free}.

By facilitating user interaction with the model’s outputs, \sysname{} supports task-specific evaluations that align with real-world applications, ensuring LMMs are assessed on technical accuracy and their ability to meet domain-specific expectations. 




% \subsection{Potential Implications and Future Directions}

% \paragraph{\textbf{Generating Pseudo-Annotations for Fine-tuning of Models}}
% One of the noteworthy implications of \sysname{} is its capability to facilitate the creation of pseudo annotations. 
% This aspect is particularly beneficial when ground truth data is limited or unavailable. 
% %
% These annotations can serve as valuable resources for further model fine-tuning, providing a pathway to improve the model's performance.
% The consistency of \sysname{}'s evaluation with established metrics such as $F_1$, as demonstrated in our study, assures the credibility of these pseudo annotations in representing the actual performance of the models.

% \subsection{{Promoting User Agency}}
% \sysname{} significantly enhances user agency by enabling individuals without specialized knowledge to effectively evaluate and interact with LMMs.
% %
% This democratization of model evaluation is pivotal, as it breaks down the technical barriers that typically limit model assessment to experts in the field.
% %
% With \sysname{}, users can directly engage with the model's outputs, make informed judgments about its performance, 
% and even influence its development through feedback loops.
% %
% This empowerment of users enhances LMM evaluation accessibility and enriches model development with diverse insights.



\subsection{{\sysname{} in Promoting User Agency}}

\sysname{} plays a crucial role in promoting user agency by empowering individuals, regardless of technical expertise, to effectively evaluate and interact with large, multi-modal AI models (LMMs). 
This democratization of model evaluation is transformative, as it dismantles the barriers that traditionally confine model assessment to a niche group of experts. By providing an intuitive visual interface, \sysname{} enables users to engage directly with the outputs of LMMs, allowing them to assess the model's performance based on their unique perspectives and needs.

This user-centered approach not only makes LMM evaluation more accessible but also enriches the development process by incorporating a wider range of insights. When users can make informed judgments about a model's reliability and relevance in specific contexts, they contribute valuable feedback that can guide the model's iterative refinement. 
This feedback loop ensures that the development of LMMs is more aligned with real-world applications and user expectations, ultimately leading to more robust and trustworthy AI systems. 








\subsection{{\sysname{} as a Complement to Automated Evaluations}}
Traditional assessments of LMMs depend on the availability of ground truth data of some capacity, such as tagged harmful, hateful, and biased content~\cite{gptv_system_card}.
%
Where ground truth is unavailable, \sysname{} provides an alternative means of evaluating LMMs. 
%
Recall that the participant ratings for different models in our study closely resemble their underlying $F_1$ scores, as demonstrated in Sec.~\ref{subsec:all_org_model_ratings}.
%
Remarkably, \sysname{} requires only a select number of video frames and objects to perform evaluations, 
yet it delivers outcomes that agree with $F_1$-scores calculated across the entire dataset.
%
Therefore, \sysname{} can be a valuable complementary framework to existing automated evaluation techniques, offering reliable insights when ground truth is unavailable.


% \subsection{Extending \sysname{} for Users with Color Blindness}
% To ensure that \sysname{} is accessible to users with color blindness, it is crucial to go beyond simple color differentiation. 
% One possible solution is introducing distinct textures or patterns in the cells instead of colors to represent different values.
% %
% For instance, diagonal stripes can represent cells where the object exists, while crosshatching can represent the ones for which an object does not exist.
% %
% This would allow users with any form of color vision deficiency, including Deuteranopia, Protanopia, and Tritanopia, to easily interpret the heatmap based on texture rather than relying on color.

% Another approach is to allow users to customize the color scheme by selecting a pair of colors they can easily distinguish. 
% Many individuals with color blindness can differentiate between certain color combinations even if they cannot perceive the entire spectrum. 
% Providing customizable color options, such as blue and orange, would allow users to tailor the visualization to their specific needs













% - visualization with GT data; 4 colors, but demanding as tracking 4 colors is hard (V1)
% - One heatmap with two colors came out as the more convenient option, which also enables analysis without GT data (V2)
% - One heatmap with objects I see and I don't see, separated by a blacked-out row in the middle. (V1)
% The issue is one heatmap with two separate color meanings
% - two heatmaps side by side, but too much information, and what if someone wants to test only one model (V2)
% - added bargraph for an overview of all modifications (V3)
% - Added litmus objects (V3)
% - synchronization among all dashboard items, such as the image container, the heatmap, and the object selection panel.
% selections were highlighted, and objects could be added/deleted dynamically as needed (V2)
% - the first version listed all the objects in a read-only textbox. Users would have to look for options from there. V2 introduced the dropdown and objects as options.
% - image popup on click in a separate window introduced (V2). Allows for detail on demand and more info later as needed

% \subsection{Components of \sysname{}}
% This section discusses each component in \sysname{}.
% The final version of \sysname{} is shown in Figure~\ref{fig:dashboard_final}.

% \paragraph{Model, Task and Video Dropdowns (A, B, C).}
% The dashboard features a Model dropdown (A) that lets users choose from various LMMs for analysis. 
% Additionally, the Task dropdown (B) allows users to select the specific task (currently only one) they wish to perform on a video, with the current option being multi-object classification in a video. 
% Lastly, the Video dropdown (C) allows users to select a specific segment for analysis.

% \paragraph{Image Container (G).}
% When a user selects a video segment from the video dropdown, the image container (G) is populated with up to 16 keyframes extracted from that segment. 
% % Each frame is labeled with a number ranging from 0 to N, where N represents the total number of frames. 
% % This numerical label is displayed in the top-left corner of each frame.
% %
% Users have the option to view a larger version of an image frame by clicking on it, which opens the operating system's default image viewer in a separate window (not shown in Figure~\ref{fig:dashboard_final}).
% This feature allows users to access additional information on demand.
% %
% Additionally, each frame in the image container features a checkbox, allowing users to exclude frames perceived as blurry, poorly visible, 
% or with unfavorable camera angles by unchecking the checkbox and reintroducing them by checking it if necessary.


% \paragraph{Object Selection Panel (D).}
% The Object Selection panel (D) is placed above the image container on the left. 
% When a video is selected, it populates with suggested objects influenced by the currently selected model, primarily drawing from the group of objects the model was originally trained on.
% %
% The last suggestion is a \emph{litmus object}, marked in violet. 
% This object are deliberately chosen to be extremely unlikely to appear in any video frames across the dataset, testing the model's accuracy in identifying their absence.
% %

% Users can add more litmus objects by typing the object's name preceded by '*.' 
% These '*'-prefixed litmus objects appear in \color{violet}{violet} \color{black}{at} the end of the selection list.
% In Figure~\ref{fig:dashboard_final}, \emph{Chair} is a litmus objects.

% % Some suggestions are randomly selected from objects outside the model's training set. 
% % Users can remove individual objects by clicking the cross icon next to each object to manage the list. Alternatively, they can clear the entire list using the large cross button near the dropdown icon.
% %
% % Note that a specific object may not be present in every video frame. Users can select objects they generally observe, even if they are not present in all frames. To facilitate this, users can begin typing the names of the objects they see, and the dropdown will suggest possible names based on the entered text.

% \paragraph{Model's Performance Summary: Binary Heatmap (E).}
% A summary of the model's performance in the selected video is shown using a heatmap (E).
% In the heatmap, the video frame numbers are along the X-axis, and the objects from D are on the Y-axis. 
% Green means the model says the object is present in a frame, and red represents the model says the object is not present.
% % For instance, in Figure~\ref{fig:dashboard_final}, \emph{Model-0} says that \emph{Traffic Signals} are present in \emph{Frame-3}, but \emph{Wet Surface} is absent.

% The user can hover over any cell in the heatmap, and the corresponding video frame will be highlighted in yellow below in the image container (G) section.
% Using the hover option, the user can verify whether the model is correct when detecting an object.


% Note that the model can make mistakes either way; 
% it can say something is there when it is not and miss something when it is in the frame.
% Thus, red and green do not mean good or bad by themselves. 
% The user needs to check a specific cell in the heatmap to decide whether the model is correct.
% %
% If the user feels the model has made any error, they can correct it by clicking on that cell.
% In other words, when a user clicks on a green cell, it turns red, and vice versa.
% A summary of all the clicks is shown in the bargraph (F) on the right of the heatmap.

% \paragraph{Modification Summary: Bargraph (F).}
% The bargraph (F) becomes visible on the right side of the heatmap (E) after the user makes at least one modification.
% Each bar in the bargraph represents the total number of modifications in a frame.
% % The primary purpose of the bargraph is to assist users in keeping track of the corrections they have made to the model's predictions.

% % For instance, in Figure~\ref{fig:dashboard_final}, there are nine rows, one for each object in the object selection panel (D).
% % If the user starts scanning the heatmap cells from the top row and makes their way down gradually, 
% % they might probably forget what they observed in the first few rows by the time they are near the end.
% % However, as the user clicks and corrects model mistakes along the way, the bargraph serves as a high-level summary of the model's performance thus far.




% \paragraph{Rating Slider (H), Comments (I), and Reset Button (J).}
% The final three components of \sysname{} include the rating slider (H), comments box (I), and the record and reset button (J).
% The slider (H) ranges from 0\% to 100\% in increments of 10\%, enabling users to select values like 10\%, 80\%, and so forth, but not intermediate values like 15\% or 85\%.
% %
% After providing a rating, users can leave comments in the comment box (I).
% In the end, they can press the \emph{Record Response and Reset} button (J) at the bottom of \sysname{}. 



